Online GentleAdaBoost -- Technical Report

We study the online variant of GentleAdaboost, where we combine a weak learner to a strong learner in an online fashion. We provide an approach to extend the batch approach to an online approach with theoretical justifications through application of line search. Finally we compare our online boosting approach with other online approaches across a variety of benchmark datasets.

==> _authors.tex <==
$-- You can use as many custom partials as you need. Convention is to prefix name with '_'
$-- It can be useful to use such template to split some template parts in smaller pieces, which is easier to reuse.
$-- This '_custom.tex' is used on 'title.tex' as example.
$-- See other existing format in quarto-journals/ organisation.
$-- %%%% TODO %%%%%
$-- Use it if you need to insert content at this specific place of the main Pandoc's template. Otherwise, remove it.
$-- Here we are using it to format the authors part of the template.
$-- %%%%%%%%%%%%%%%

\textbf{$it.name.literal$}$if(it.orcid)$~\orcidlink{$it.orcid$}$endif$$for(it.affiliations/first)$\\$it.department$\\$it.name$\\$if(it.city)$$it.city$$if(it.postal-code)$,\ $it.postal-code$$endif$$endif$$endfor$\\$if(it.email)$\href{mailto:$it.email$}{$it.email$}$endif$


==> before-body.tex <==
$-- Implements the frontmatter, title page, and abstract.
$--
$-- %%%% TODO %%%%%
$-- Customize is needed, otherwise remove this partials to use Quarto default one
$-- %%%%%%%%%%%%%%%%
$if(has-frontmatter)$
\frontmatter
$endif$
$if(title)$
$if(beamer)$
\frame{\titlepage}
$else$
\maketitle
$endif$
$if(abstract)$
\begin{abstract}
$abstract$
\end{abstract}
$endif$
$endif$
$if(keywords)$
{\bfseries \emph Keywords}
\def\sep{\textbullet\ }
$for(keywords/allbutlast)$$keywords$ \sep $endfor$
$for(keywords/last)$$keywords$$endfor$

$endif$


==> title.tex <==
$-- Provides configuration of document metadata for writing the title block.
$-- Note that in addition to these templates and partials, Quarto will also make normalized authors and affiliations data available to the template,
$-- making is easy to write custom title blocks against a standard schema.
$--
$-- %%%% TODO %%%%%
$-- Customize is needed, like below for printing the authors. Otherwise remove this partials to use Quarto default one.
$-- %%%%%%%%%%%%%%%%
$if(linenumbers)$
\usepackage{lineno}
\linenumbers
$endif$
$if(doublespacing)$
\usepackage{setspace}
\doublespacing
$endif$
\newcommand{\runninghead}{A Preprint }
$if(runninghead)$
\renewcommand{\runninghead}{$runninghead$ }
$endif$
$if(title)$
\title{$title$$if(thanks)$\thanks{$thanks$}$endif$}
$endif$
$if(subtitle)$
\usepackage{etoolbox}
\makeatletter
\providecommand{\subtitle}[1]{% add subtitle to \maketitle
  \apptocmd{\@title}{\par {\large #1 \par}}{}{}
}
\makeatother
\subtitle{$subtitle$}
$endif$
\author{${ by-author:_authors.tex()[\\\\\\] }}


